Developments and applications of the OPTIMADE API for materials discovery, design, and data exchange

The Open Databases Integration for Materials Design (OPTIMADE) application programming interface (API) empowers users with holistic access to a growing federation of databases, enhancing the accessibility and discoverability of materials and chemical data. Since the first release of the OPTIMADE specification (v1.0), the API has undergone significant development, leading to the upcoming v1.2 release, and has underpinned multiple scientific studies. In this work, we highlight the latest features of the API format, accompanying software tools, and provide an update on the implementation of OPTIMADE in contributing materials databases. We end by providing several use cases that demonstrate the utility of the OPTIMADE API in materials research that continue to drive its ongoing development.

==> table_redux_diff.tex <==
\begin{table*}[t]
\centering
\ttfamily
\small{
\begin{tabular}{l|rrrr}
\bf{\texttt{PROVIDER}}&\bf{N$_1$}&\bf{N$_2$}&\bf{N$_3$}&\bf{N\textsubscript{tot}}\\
\hline
AFLOW & \href{http://aflow.org/API/optimade/v1/structures?filter=elements%20HAS%20ANY%20%22C%22%2C%22Si%22%2C%22Ge%22%2C%22Sn%22%2C%22Pb%22}{704,302} ({700,192}) & \href{http://aflow.org/API/optimade/v1/structures?filter=elements%20HAS%20ANY%20%22C%22%2C%22Si%22%2C%22Ge%22%2C%22Sn%22%2C%22Pb%22%20AND%20nelements%3D2}{63,017} ({62,293}) & \href{http://aflow.org/API/optimade/v1/structures?filter=elements%20HAS%20ANY%20%22C%22%2C%22Si%22%2C%22Ge%22%2C%22Sn%22%20AND%20NOT%20elements%20HAS%20%22Pb%22%20AND%20elements%20LENGTH%203}{413,797} ({382,554}) & \href{http://aflow.org/API/optimade/v1/structures?filter=nelements>=1}{3,530,330} \\
Alexandria$^\star$ & \href{https://alexandria.icams.rub.de/pbe/v1/structures?filter=elements%20HAS%20ANY%20%22C%22%2C%22Si%22%2C%22Ge%22%2C%22Sn%22%2C%22Pb%22}{939,084} & \href{https://alexandria.icams.rub.de/pbe/v1/structures?filter=elements%20HAS%20ANY%20%22C%22%2C%22Si%22%2C%22Ge%22%2C%22Sn%22%2C%22Pb%22%20AND%20nelements%3D2}{48,510} & \href{https://alexandria.icams.rub.de/pbe/v1/structures?filter=elements%20HAS%20ANY%20%22C%22%2C%22Si%22%2C%22Ge%22%2C%22Sn%22%20AND%20NOT%20elements%20HAS%20%22Pb%22%20AND%20elements%20LENGTH%203}{437,768} & \href{https://alexandria.icams.rub.de/pbe/v1/structures?filter=nelements>=1}{5,055,842} \\
COD & \href{https://www.crystallography.net/cod/optimade/v1/structures?filter=elements%20HAS%20ANY%20%22C%22%2C%22Si%22%2C%22Ge%22%2C%22Sn%22%2C%22Pb%22}{458,249} ({416,314}) & \href{https://www.crystallography.net/cod/optimade/v1/structures?filter=elements%20HAS%20ANY%20%22C%22%2C%22Si%22%2C%22Ge%22%2C%22Sn%22%2C%22Pb%22%20AND%20nelements%3D2}{4,082} ({3,896}) & \href{https://www.crystallography.net/cod/optimade/v1/structures?filter=elements%20HAS%20ANY%20%22C%22%2C%22Si%22%2C%22Ge%22%2C%22Sn%22%20AND%20NOT%20elements%20HAS%20%22Pb%22%20AND%20elements%20LENGTH%203}{34,739} ({32,420}) & \href{https://www.crystallography.net/cod/optimade/v1/structures?filter=nelements>=1}{512,282} \\
CMR & \href{https://cmr-optimade.fysik.dtu.dk/v1/structures?filter=elements%20HAS%20ANY%20%22C%22%2C%22Si%22%2C%22Ge%22%2C%22Sn%22%2C%22Pb%22}{147} & \href{https://cmr-optimade.fysik.dtu.dk/v1/structures?filter=elements%20HAS%20ANY%20%22C%22%2C%22Si%22%2C%22Ge%22%2C%22Sn%22%2C%22Pb%22%20AND%20nelements%3D2}{147} & \href{https://cmr-optimade.fysik.dtu.dk/v1/structures?filter=elements%20HAS%20ANY%20%22C%22%2C%22Si%22%2C%22Ge%22%2C%22Sn%22%20AND%20NOT%20elements%20HAS%20%22Pb%22%20AND%20elements%20LENGTH%203}{0} & \href{https://cmr-optimade.fysik.dtu.dk/v1/structures?filter=nelements>=1}{1,536} \\
% MatCloud & \href{}{0} & \href{}{0} & \href{}{0} & \href{}{0} \\

JARVIS-DFT & \href{https://jarvis.nist.gov/optimade/jarvisdft/v1/structures/?filter=elements HAS ANY "C", "Si", "Ge", "Sn", "Pb"}{9,017} & \href{https://jarvis.nist.gov/optimade/jarvisdft/v1/structures/?filter=elements HAS ANY "C", "Si", "Ge", "Sn", "Pb" AND nelements=2}{1,426} & \href{
https://jarvis.nist.gov/optimade/jarvisdft/v1/structures/?filter=elements HAS ANY "C", "Si", "Ge", "Sn", AND NOT elements HAS "Pb" AND elements LENGTH 3}{8,084}  & \href{https://jarvis.nist.gov/optimade/jarvisdft/v1/structures/?filter=nelements%3E=1}{77,096} \\

Materials Cloud$^\star$ & \href{https://aiida.materialscloud.org/optimade-sample/optimade/v1/structures?filter=elements%20HAS%20ANY%20%22C%22%2C%22Si%22%2C%22Ge%22%2C%22Sn%22%2C%22Pb%22}{961,564} & \href{https://aiida.materialscloud.org/optimade-sample/optimade/v1/structures?filter=elements%20HAS%20ANY%20%22C%22%2C%22Si%22%2C%22Ge%22%2C%22Sn%22%2C%22Pb%22%20AND%20nelements%3D2}{4,218} & \href{https://aiida.materialscloud.org/optimade-sample/optimade/v1/structures?filter=elements%20HAS%20ANY%20%22C%22%2C%22Si%22%2C%22Ge%22%2C%22Sn%22%20AND%20NOT%20elements%20HAS%20%22Pb%22%20AND%20elements%20LENGTH%203}{136,176} & \href{https://aiida.materialscloud.org/optimade-sample/optimade/v1/structures?filter=nelements>=1}{4,515,120} \\
Materials Project & \href{https://optimade.materialsproject.org/v1/structures/?filter=elements HAS ANY "C", "Si", "Ge", "Sn", "Pb"}{34,424} (27,309) & \href{https://optimade.materialsproject.org/v1/structures/?filter=elements HAS ANY "C", "Si", "Ge", "Sn", "Pb" AND nelements=2}{3,750} (3,545) & \href{https://optimade.materialsproject.org/v1/structures/?filter=elements HAS ANY "C", "Si", "Ge", "Sn", AND NOT elements HAS "Pb" AND elements LENGTH 3}{11,861} (10,501) & \href{https://optimade.materialsproject.org/v1/structures}{154,387} \\
MPDD & \href{http://mpddoptimade.phaseslab.org/v1/structures?filter=elements%20HAS%20ANY%20%22C%22%2C%22Si%22%2C%22Ge%22%2C%22Sn%22%2C%22Pb%22}{811,136} & \href{http://mpddoptimade.phaseslab.org/v1/structures?filter=elements%20HAS%20ANY%20%22C%22%2C%22Si%22%2C%22Ge%22%2C%22Sn%22%2C%22Pb%22%20AND%20nelements%3D2}{80,195} & \href{http://mpddoptimade.phaseslab.org/v1/structures?filter=elements%20HAS%20ANY%20%22C%22%2C%22Si%22%2C%22Ge%22%2C%22Sn%22%20AND%20NOT%20elements%20HAS%20%22Pb%22%20AND%20elements%20LENGTH%203}{490,900} & \href{http://mpddoptimade.phaseslab.org/v1/structures?filter=nelements>=1}{3,975,666} \\
MPOD & \href{http://mpod_optimade.cimav.edu.mx/v1/structures?filter=elements%20HAS%20ANY%20%22C%22%2C%22Si%22%2C%22Ge%22%2C%22Sn%22%2C%22Pb%22}{91} & \href{http://mpod_optimade.cimav.edu.mx/v1/structures?filter=elements%20HAS%20ANY%20%22C%22%2C%22Si%22%2C%22Ge%22%2C%22Sn%22%2C%22Pb%22%20AND%20nelements%3D2}{8} & \href{http://mpod_optimade.cimav.edu.mx/v1/structures?filter=elements%20HAS%20ANY%20%22C%22%2C%22Si%22%2C%22Ge%22%2C%22Sn%22%20AND%20NOT%20elements%20HAS%20%22Pb%22%20AND%20elements%20LENGTH%203}{16} & \href{http://mpod_optimade.cimav.edu.mx/v1/structures?filter=nelements>=1}{401} \\
MPDS & \href{https://api.mpds.io/v1/structures?filter=elements%20HAS%20ANY%20%22C%22%2C%22Si%22%2C%22Ge%22%2C%22Sn%22%2C%22Pb%22}{-} & \href{https://api.mpds.io/v1/structures?filter=elements%20HAS%20ANY%20%22C%22%2C%22Si%22%2C%22Ge%22%2C%22Sn%22%2C%22Pb%22%20AND%20nelements%3D2}{-} & \href{https://api.mpds.io/v1/structures?filter=elements%20HAS%20ANY%20%22C%22%2C%22Si%22%2C%22Ge%22%2C%22Sn%22%20AND%20NOT%20elements%20HAS%20%22Pb%22%20AND%20elements%20LENGTH%203}{-} & \href{https://api.mpds.io/v1/structures?filter=nelements>=1}{507,178} \\
NOMAD & \href{https://nomad-lab.eu/prod/rae/optimade/v1/structures?filter=elements%20HAS%20ANY%20%22C%22%2C%22Si%22%2C%22Ge%22%2C%22Sn%22%2C%22Pb%22}{4,451,056} ({3,359,594}) & \href{https://nomad-lab.eu/prod/rae/optimade/v1/structures?filter=elements%20HAS%20ANY%20%22C%22%2C%22Si%22%2C%22Ge%22%2C%22Sn%22%2C%22Pb%22%20AND%20nelements%3D2}{587,923} ({532,123}) & \href{https://nomad-lab.eu/prod/rae/optimade/v1/structures?filter=elements%20HAS%20ANY%20%22C%22%2C%22Si%22%2C%22Ge%22%2C%22Sn%22%20AND%20NOT%20elements%20HAS%20%22Pb%22%20AND%20elements%20LENGTH%203}{2,092,989} ({1,611,302}) & \href{https://nomad-lab.eu/prod/rae/optimade/v1/structures?filter=nelements>=1}{12,116,021} \\
\emph{odbx}$^\star$ & \href{https://optimade-misc.odbx.science/v1/structures?filter=elements%20HAS%20ANY%20%22C%22%2C%22Si%22%2C%22Ge%22%2C%22Sn%22%2C%22Pb%22}{125,648} ({55}) & \href{https://optimade-misc.odbx.science/v1/structures?filter=elements%20HAS%20ANY%20%22C%22%2C%22Si%22%2C%22Ge%22%2C%22Sn%22%2C%22Pb%22%20AND%20nelements%3D2}{3,179} ({54}) & \href{https://optimade-misc.odbx.science/v1/structures?filter=elements%20HAS%20ANY%20%22C%22%2C%22Si%22%2C%22Ge%22%2C%22Sn%22%20AND%20NOT%20elements%20HAS%20%22Pb%22%20AND%20elements%20LENGTH%203}{17,009} ({0}) & \href{https://optimade-misc.odbx.science/v1/structures?filter=nelements>=1}{523,216} \\
\emph{omdb} & \href{http://optimade.openmaterialsdb.se/v1/structures?filter=elements%20HAS%20ANY%20%22C%22%2C%22Si%22%2C%22Ge%22%2C%22Sn%22%2C%22Pb%22}{58,718} ({58,718}) & \href{http://optimade.openmaterialsdb.se/v1/structures?filter=elements%20HAS%20ANY%20%22C%22%2C%22Si%22%2C%22Ge%22%2C%22Sn%22%2C%22Pb%22%20AND%20nelements%3D2}{690} ({690}) & \href{http://optimade.openmaterialsdb.se/v1/structures?filter=elements%20HAS%20ANY%20%22C%22%2C%22Si%22%2C%22Ge%22%2C%22Sn%22%20AND%20NOT%20elements%20HAS%20%22Pb%22%20AND%20elements%20LENGTH%203}{7,428} ({7,428}) & \href{http://optimade.openmaterialsdb.se/v1/structures?filter=nelements>=1}{68,566} \\
OQMD & \href{http://oqmd.org/optimade/v1/structures?filter=elements%20HAS%20ANY%20%22C%22%2C%22Si%22%2C%22Ge%22%2C%22Sn%22%2C%22Pb%22}{261,400} ({153,113}) & \href{http://oqmd.org/optimade/v1/structures?filter=elements%20HAS%20ANY%20%22C%22%2C%22Si%22%2C%22Ge%22%2C%22Sn%22%2C%22Pb%22%20AND%20nelements%3D2}{15,375} ({11,011}) & \href{http://oqmd.org/optimade/v1/structures?filter=elements%20HAS%20ANY%20%22C%22%2C%22Si%22%2C%22Ge%22%2C%22Sn%22%20AND%20NOT%20elements%20HAS%20%22Pb%22%20AND%20elements%20LENGTH%203}{81,673} ({70,252}) & \href{http://oqmd.org/optimade/v1/structures?filter=nelements>=1}{1,226,781} \\
TCOD & \href{https://www.crystallography.net/tcod/optimade/v1/structures?filter=elements%20HAS%20ANY%20%22C%22%2C%22Si%22%2C%22Ge%22%2C%22Sn%22%2C%22Pb%22}{7,161} ({2,631}) & \href{https://www.crystallography.net/tcod/optimade/v1/structures?filter=elements%20HAS%20ANY%20%22C%22%2C%22Si%22%2C%22Ge%22%2C%22Sn%22%2C%22Pb%22%20AND%20nelements%3D2}{296} ({296}) & \href{https://www.crystallography.net/tcod/optimade/v1/structures?filter=elements%20HAS%20ANY%20%22C%22%2C%22Si%22%2C%22Ge%22%2C%22Sn%22%20AND%20NOT%20elements%20HAS%20%22Pb%22%20AND%20elements%20LENGTH%203}{662} ({660}) & \href{https://www.crystallography.net/tcod/optimade/v1/structures?filter=nelements>=1}{7,452} \\
2DMatpedia & \href{http://optimade.2dmatpedia.org/v1/structures?filter=elements%20HAS%20ANY%20%22C%22%2C%22Si%22%2C%22Ge%22%2C%22Sn%22%2C%22Pb%22}{1,172} & \href{http://optimade.2dmatpedia.org/v1/structures?filter=elements%20HAS%20ANY%20%22C%22%2C%22Si%22%2C%22Ge%22%2C%22Sn%22%2C%22Pb%22%20AND%20nelements%3D2}{739} & \href{http://optimade.2dmatpedia.org/v1/structures?filter=elements%20HAS%20ANY%20%22C%22%2C%22Si%22%2C%22Ge%22%2C%22Sn%22%20AND%20NOT%20elements%20HAS%20%22Pb%22%20AND%20elements%20LENGTH%203}{255} & \href{http://optimade.2dmatpedia.org/v1/structures?filter=nelements>=1}{6,351} \\
\end{tabular}
}
\caption{The table from Ref.~\cite{OPTIMADE2021} recreated in \DIFaddbeginFL \DIFaddFL{March }\DIFaddendFL 2024, with new providers. \DIFaddbeginFL \DIFaddFL{The final column indicates the total number of structures served by each OPTIMADE API.  }\DIFaddendFL Providers that serve multiple databases are indicated with $\star$\DIFaddbeginFL \DIFaddFL{. Results for Materials Cloud and Materials Cloud Archive have been aggregated under the same title}\DIFaddendFL . The corresponding values from the 2021 paper \cite{OPTIMADE2021} are provided in brackets, where appropriate.}
\label{tab:table_redux}
\end{table*}

